DUnE: Dataset for Unified Editing

Even the most advanced language models remain susceptible to errors necessitating to modify these models without initiating a comprehensive retraining process. Model editing refers to the modification of a model's knowledge or representations in a manner that produces the desired outcomes. Prior research primarily centered around editing factual data e.g. "Messi plays for Inter Miami" confining the definition of an edit to a knowledge triplet i.e. (subject, object, relation). However, as the applications of language models expand, so do the diverse ways in which we wish to edit and refine their outputs. In this study, we broaden the scope of the editing problem to include an array of editing cases such as debiasing and rectifying reasoning errors and define an edit as any natural language expression that solicits a change in the model's outputs. We are introducing DUnE-an editing benchmark where edits are natural language sentences and propose that DUnE presents a challenging yet relevant task. To substantiate this claim, we conduct an extensive series of experiments testing various editing approaches to address DUnE, demonstrating their respective strengths and weaknesses. We show that retrieval-augmented language modeling can outperform specialized editing techniques and neither set of approaches has fully solved the generalized editing problem covered by our benchmark.

==> background.tex <==
Define Format-Free Editing problem using notation, what is an edit, what is the test inputs what does it fix.
Desiderata: Reliability, Consistency, Locality, Reversibility.

==> tables/results_consistency.tex <==
\begin{table*}[t]
    \centering
    \caption{Results on for \dune evaluation examples. Proprietary models Bard, GPT-3.5 and GPT-4 are not available for fine-tuning. Scores that are closest to \textit{Gold Edit-in-Context} are highlighted when better than \textit{Before-Editing}.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c}
    \vspace{0.5cm} % Vertical spacing
        \begin{subtable}{1.3\linewidth}
            \centering
            \caption{Adding New Information}
            \begin{tabular}{lcccccccc}
            \toprule
            \multirow{3}{*}{\bf Technique} & \multicolumn{8}{c}{\bf Models} \\ \cmidrule{2-9}
            & \bf Flan-T5-Small & \bf  Flan-T5-Base & \bf  Flan-T5-Large & \bf  Flan-T5-XL & \bf  Flan-T5-XXL & \bf  GPT-3.5 & \bf  GPT-4 & \bf Bard \\ \midrule
            Before-Editing               &           28.5 &          27.4 &           37.9 &        37.1 &         37.4 &    39.9 &  57.8 &  68.6 \\
Fine-Tuning           &           36.1 &          22.1 &           20.4 &        30.3 &         32.2 &       - &     - &     - \\
GPT-3 Embeddings      &           38.1 &          40.4 &           51.3 &        51.1 &         47.6 &    38.2 &  43.9 &   70.1 \\
SERAC &           29.7 &          29.2 &           41.4 &        40.3 &         37.7 &    33.7 &  42.3 &  69.4 \\
BM25             &           \textbf{89.0} &          \textbf{96.0} &           \textbf{96.7} &       \textbf{ 97.1} &         \textbf{96.2} &    \textbf{73.6} &  \textbf{79.2} &  \textbf{97.5} \\
\textit{Gold Edit-in-Context}  &           90.9 &          98.5 &           98.4 &        98.9 &         98.5 &    75.2 &  80.4 &  98.7 \\ \bottomrule
            \end{tabular}
            \label{tab:sub_newinfo}
        \end{subtable}
        \\
        \begin{subtable}{1.3\linewidth}
            \centering
            \caption{Arithmetic Reasoning}
            \begin{tabular}{lcccccccc}
            \toprule
            \multirow{3}{*}{\bf Technique} & \multicolumn{8}{c}{\bf Models} \\ \cmidrule{2-9}
            & \bf Flan-T5-Small & \bf Flan-T5-Base & \bf  Flan-T5-Large & \bf  Flan-T5-XL & \bf  Flan-T5-XXL & \bf  GPT-3.5 & \bf  GPT-4 & \bf Bard \\ \midrule
            Before-Editing               &            0.8 &           0.9 &            1.0 &         1.3 &          8.6 &    87.8 &  90.0 &  82.9 \\
Fine-Tuning           &            0.8 &           0.7 &            0.4 &         2.0 &         11.6 &       - &     - &     - \\
GPT-3 Embeddings      &            1.1 &           1.4 &            6.8 &         9.0 &         12.5 & 78.5 &  89.8 &  83.1 \\
SERAC &            \textbf{2.7} &           \textbf{6.3} &           \textbf{23.8} &        \textbf{36.2} &         \textbf{43.9} &    87.7 &  90.0 &  \textbf{88.1} \\
BM25             &            0.7 &           1.7 &            3.7 &         6.4 &         13.5 &    87.7 &  90.0 &  83.1 \\
\textit{Gold Edit-in-Context}  &            5.7 &          12.4 &           56.2 &        84.8 &         95.5 &    90.3 &  96.2 &  99.4 \\ \bottomrule
            \end{tabular}
            \label{tab:sub_arithmetic}
        \end{subtable}
        \vspace{0.5cm} % Vertical spacing
        \\
        \begin{subtable}{1.3\linewidth}
            \centering
            \caption{Scientific Reasoning}
            \begin{tabular}{lcccccccc}
            \toprule
            \multirow{3}{*}{\bf Technique} & \multicolumn{8}{c}{\bf Models} \\ \cmidrule{2-9}
            & \bf  Flan-T5-Small & \bf  Flan-T5-Base & \bf  Flan-T5-Large & \bf  Flan-T5-XL & \bf Flan-T5-XXL & \bf GPT-3.5 & \bf GPT-4 & \bf Bard \\ \midrule
            Before-Editing               &           38.0 &          53.2 &           67.0 &        76.1 &         79.8 &    88.2 &  87.8 &  84.9 \\
Fine-Tuning           &           34.3 &          35.1 &           59.5 &        74.7 &         78.2 &       - &     - &     - \\
GPT-3 Embeddings      &           38.1 &          52.5 &           66.4 &        75.1 &         80.3 &    87.1 &  88.3 &  83.5 \\
SERAC &           39.0 &          54.0 &           67.5 &        76.3 &         80.2 &    87.7 &  88.1 &  85.3 \\
BM25             &          \textbf{ 52.7 }&          \textbf{65.6} &          \textbf{ 74.7} &        \textbf{82.0} &        \textbf{ 84.7} &    \textbf{90.3} &  \textbf{89.9} & \textbf{ 87.5} \\
\textit{Gold Edit-in-Context}  &           54.6 &          67.6 &           75.4 &        82.8 &         85.7 &    92.0 &  90.6 &  88.8 \\ \bottomrule
            \end{tabular}
            \label{tab:sub_reasoning}
        \end{subtable}
    \end{tabular}
    }\label{tab:main_results}
\end{table*}



